The Construction of Large-scale Structure Catalogs for the Dark Energy Spectroscopic Instrument

We present the technical details on how large-scale structure (LSS) catalogs are constructed from redshifts measured from spectra observed by the Dark Energy Spectroscopic Instrument (DESI). The LSS catalogs provide the information needed to determine the relative number density of DESI tracers as a function of redshift and celestial coordinates and, e.g., determine clustering statistics. We produce catalogs that are weighted subsamples of the observed data, each matched to a weighted `random' catalog that forms an unclustered sampling of the probability density that DESI could have observed those data at each location. Precise knowledge of the DESI observing history and associated hardware performance allows for a determination of the DESI footprint and the number of times DESI has covered it at sub-arcsecond level precision. This enables the completeness of any DESI sample to be modeled at this same resolution. The pipeline developed to create LSS catalogs has been designed to easily allow robustness tests and enable future improvements. We describe how it allows ongoing work improving the match between galaxy and random catalogs, such as including further information when assigning redshifts to randoms, accounting for fluctuations in target density, accounting for variation in the redshift success rate, and accommodating blinding schemes.

==> figures/DESI-2024-0402_author_list.tex <==
% Author list file generated with: mkauthlist 1.3.0+14.gcc6daf1.dirty 
% mkauthlist -f --sort-firsttier --orcid -j jcap DESI-2024-0402_author_list.csv DESI-2024-0402_author_list.tex 
%% Orcid numbers may need \usepackage{orcidlink}.
%% Use \input to call the file


\author[1]{{A.~J.~Ross}\orcidlink{0000-0002-7522-9083},}
\author[2]{{J.~Aguilar},}
\author[3]{{S.~Ahlen}\orcidlink{0000-0001-6098-7247},}
\author[4]{{S.~Alam}\orcidlink{0000-0002-3757-6359},}
\author[2]{{A.~Anand}\orcidlink{0000-0003-2923-1585},}
\author[2]{{S.~Bailey}\orcidlink{0000-0003-4162-6619},}
\author[5]{{D.~Bianchi}\orcidlink{0000-0001-9712-0006},}
\author[6]{{S.~Brieden}\orcidlink{0000-0003-3896-9215},}
\author[7]{{D.~Brooks},}
\author[8]{{E.~Burtin},}
\author[9,10]{{A.~Carnero Rosell}\orcidlink{0000-0003-3044-5150},}
\author[2]{{E.~Chaussidon}\orcidlink{0000-0001-8996-4874},}
\author[2]{{T.~Claybaugh},}
\author[11]{{S.~Cole}\orcidlink{0000-0002-5954-7903},}
\author[12]{{K.~Dawson},}
\author[13]{{A.~de la Macorra}\orcidlink{0000-0002-1769-1640},}
\author[8]{{A.~de~Mattia},}
\author[14]{{Arjun~Dey}\orcidlink{0000-0002-4928-4003},}
\author[15]{{Biprateep~Dey}\orcidlink{0000-0002-5665-7912},}
\author[7]{{P.~Doel},}
\author[16,17]{{K.~Fanning}\orcidlink{0000-0003-2371-3356},}
\author[2,18]{{S.~Ferraro}\orcidlink{0000-0003-4992-7854},}
\author[19]{{J.~Ereza}\orcidlink{0000-0002-0194-4017},}
\author[7,20]{{A.~Font-Ribera}\orcidlink{0000-0002-3033-7312},}
\author[21,22]{{J.~E.~Forero-Romero}\orcidlink{0000-0002-2890-3725},}
\author[23,24,25]{{E.~Gaztañaga},}
\author[26,23,27]{{H.~Gil-Mar\'in}\orcidlink{0000-0003-0265-6217},}
\author[2]{{S.~Gontcho A Gontcho}\orcidlink{0000-0003-3142-233X},}
\author[28,29]{{A.~X.~Gonzalez-Morales}\orcidlink{0000-0003-4089-6924},}
\author[2]{{J.~Guy}\orcidlink{0000-0001-9822-6793},}
\author[30]{{C.~Hahn}\orcidlink{0000-0003-1197-0902},}
\author[31]{{S.~Heydenreich},}
\author[1,32,33]{{K.~Honscheid},}
\author[34]{{C.~Howlett}\orcidlink{0000-0002-1081-9410},}
\author[35,36]{{T.~Karim}\orcidlink{0000-0002-5652-8870},}
\author[37]{{D.~Kirkby}\orcidlink{0000-0002-8828-5463},}
\author[20,33]{{H.~Kong},}
\author[2]{{A.~Kremin}\orcidlink{0000-0001-6356-7424},}
\author[38,39,40]{{A.~Krolewski},}
\author[2]{{M.~Landriau}\orcidlink{0000-0003-1838-8528},}
\author[41]{{J.~Lasker}\orcidlink{0000-0003-2999-4873},}
\author[42]{{L.~Le~Guillou}\orcidlink{0000-0001-7178-8868},}
\author[2]{{M.~E.~Levi}\orcidlink{0000-0003-1887-1018},}
\author[43,20]{{M.~Manera}\orcidlink{0000-0003-4962-8934},}
\author[1,44,33]{{P.~Martini}\orcidlink{0000-0002-4279-4182},}
\author[2]{{P.~McDonald}\orcidlink{0000-0001-8346-8394},}
\author[14]{{A.~Meisner}\orcidlink{0000-0002-1125-7384},}
\author[45,20]{{R.~Miquel},}
\author[46]{{J.~Moon},}
\author[47]{{J.~Moustakas}\orcidlink{0000-0002-2733-4559},}
\author[13]{{A.~Muñoz-Gutiérrez},}
\author[48]{{A.~D.~Myers},}
\author[24]{{S.~Nadathur}\orcidlink{0000-0001-9070-3102},}
\author[48]{{L.~Napolitano}\orcidlink{0000-0002-5166-8671},}
\author[15]{{J.~ A.~Newman}\orcidlink{0000-0001-8684-2222},}
\author[49]{{J.~Nie}\orcidlink{0000-0001-6590-8122},}
\author[29,50]{{G.~Niz}\orcidlink{0000-0002-1544-8946},}
\author[38,39,40]{{W.~J.~Percival}\orcidlink{0000-0002-0644-5727},}
\author[2,51,18]{{C.~Poppett},}
\author[19]{{F.~Prada}\orcidlink{0000-0001-7145-8674},}
\author[2]{{A.~Raichoor}\orcidlink{0000-0001-5999-7923},}
\author[52,8,53]{{C.~Ravoux}\orcidlink{0000-0002-3500-6635},}
\author[54]{{M.~Rezaie}\orcidlink{0000-0001-5589-7116},}
\author[55]{{A.~Rosado-Marin},}
\author[56]{{G.~Rossi},}
\author[57,54,58]{{L.~Samushia}\orcidlink{0000-0002-1609-5687},}
\author[59]{{E.~Sanchez}\orcidlink{0000-0002-9646-8198},}
\author[60]{{E.~F.~Schlafly}\orcidlink{0000-0002-3569-7421},}
\author[2]{{D.~Schlegel},}
\author[55]{{H.~Seo}\orcidlink{0000-0002-6588-3508},}
\author[11]{{A.~Smith}\orcidlink{0000-0002-3712-6892},}
\author[14]{{D.~Sprayberry},}
\author[61]{{G.~Tarl\'{e}}\orcidlink{0000-0003-1704-0781},}
\author[55]{{D.~Valcin}\orcidlink{0000-0003-0129-0620},}
\author[13]{{M.~Vargas-Maga\~na}\orcidlink{0000-0003-3841-1836},}
\author[14]{{B.~A.~Weaver},}
\author[62]{{J.~Yu}\orcidlink{0009-0001-7217-8006},}
\author[42]{{P.~Zarrouk}\orcidlink{0000-0002-7305-9578},}
\author[63]{{C.~Zhao}\orcidlink{0000-0002-1991-7295},}
\author[2]{{R.~Zhou}\orcidlink{0000-0001-5381-4372},}
\author[49]{{H.~Zou}\orcidlink{0000-0002-6684-3997},}

\affiliation[1]{Center for Cosmology and AstroParticle Physics, The Ohio State University, 191 West Woodruff Avenue, Columbus, OH 43210, USA}
\affiliation[2]{Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA}
\affiliation[3]{Physics Dept., Boston University, 590 Commonwealth Avenue, Boston, MA 02215, USA}
\affiliation[4]{Tata Institute of Fundamental Research, Homi Bhabha Road, Mumbai 400005, India}
\affiliation[5]{Dipartimento di Fisica ``Aldo Pontremoli'', Universit\`a degli Studi di Milano, Via Celoria 16, I-20133 Milano, Italy}
\affiliation[6]{Institute for Astronomy, University of Edinburgh, Royal Observatory, Blackford Hill, Edinburgh EH9 3HJ, UK}
\affiliation[7]{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\affiliation[8]{IRFU, CEA, Universit\'{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affiliation[9]{Departamento de Astrof\'{\i}sica, Universidad de La Laguna (ULL), E-38206, La Laguna, Tenerife, Spain}
\affiliation[10]{Instituto de Astrof\'{\i}sica de Canarias, C/ V\'{\i}a L\'{a}ctea, s/n, E-38205 La Laguna, Tenerife, Spain}
\affiliation[11]{Institute for Computational Cosmology, Department of Physics, Durham University, South Road, Durham DH1 3LE, UK}
\affiliation[12]{Department of Physics and Astronomy, The University of Utah, 115 South 1400 East, Salt Lake City, UT 84112, USA}
\affiliation[13]{Instituto de F\'{\i}sica, Universidad Nacional Aut\'{o}noma de M\'{e}xico,  Cd. de M\'{e}xico  C.P. 04510,  M\'{e}xico}
\affiliation[14]{NSF NOIRLab, 950 N. Cherry Ave., Tucson, AZ 85719, USA}
\affiliation[15]{Department of Physics \& Astronomy and Pittsburgh Particle Physics, Astrophysics, and Cosmology Center (PITT PACC), University of Pittsburgh, 3941 O'Hara Street, Pittsburgh, PA 15260, USA}
\affiliation[16]{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Menlo Park, CA 94305, USA}
\affiliation[17]{SLAC National Accelerator Laboratory, Menlo Park, CA 94305, USA}
\affiliation[18]{University of California, Berkeley, 110 Sproul Hall \#5800 Berkeley, CA 94720, USA}
\affiliation[19]{Instituto de Astrof\'{i}sica de Andaluc\'{i}a (CSIC), Glorieta de la Astronom\'{i}a, s/n, E-18008 Granada, Spain}
\affiliation[20]{Institut de F\'{i}sica d’Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra Barcelona, Spain}
\affiliation[21]{Departamento de F\'isica, Universidad de los Andes, Cra. 1 No. 18A-10, Edificio Ip, CP 111711, Bogot\'a, Colombia}
\affiliation[22]{Observatorio Astron\'omico, Universidad de los Andes, Cra. 1 No. 18A-10, Edificio H, CP 111711 Bogot\'a, Colombia}
\affiliation[23]{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation[24]{Institute of Cosmology and Gravitation, University of Portsmouth, Dennis Sciama Building, Portsmouth, PO1 3FX, UK}
\affiliation[25]{Institute of Space Sciences, ICE-CSIC, Campus UAB, Carrer de Can Magrans s/n, 08913 Bellaterra, Barcelona, Spain}
\affiliation[26]{Departament de F\'{\i}sica Qu\`{a}ntica i Astrof\'{\i}sica, Universitat de Barcelona, Mart\'{\i} i Franqu\`{e}s 1, E08028 Barcelona, Spain}
\affiliation[27]{Institut de Ci\`encies del Cosmos (ICCUB), Universitat de Barcelona (UB), c. Mart\'i i Franqu\`es, 1, 08028 Barcelona, Spain.}
\affiliation[28]{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Av. Insurgentes Sur 1582. Colonia Cr\'{e}dito Constructor, Del. Benito Ju\'{a}rez C.P. 03940, M\'{e}xico D.F. M\'{e}xico}
\affiliation[29]{Departamento de F\'{i}sica, Universidad de Guanajuato - DCI, C.P. 37150, Leon, Guanajuato, M\'{e}xico}
\affiliation[30]{Department of Astrophysical Sciences, Princeton University, Princeton NJ 08544, USA}
\affiliation[31]{Department of Astronomy and Astrophysics, UCO/Lick Observatory, University of California, 1156 High Street, Santa Cruz, CA 95064, USA}
\affiliation[32]{Department of Physics, The Ohio State University, 191 West Woodruff Avenue, Columbus, OH 43210, USA}
\affiliation[33]{The Ohio State University, Columbus, 43210 OH, USA}
\affiliation[34]{School of Mathematics and Physics, University of Queensland, 4072, Australia}
\affiliation[35]{Center for Astrophysics $|$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA}
\affiliation[36]{Department of Astronomy \& Astrophysics, University of Toronto, Toronto, ON M5S 3H4, Canada}
\affiliation[37]{Department of Physics and Astronomy, University of California, Irvine, 92697, USA}
\affiliation[38]{Department of Physics and Astronomy, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada}
\affiliation[39]{Perimeter Institute for Theoretical Physics, 31 Caroline St. North, Waterloo, ON N2L 2Y5, Canada}
\affiliation[40]{Waterloo Centre for Astrophysics, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada}
\affiliation[41]{Department of Physics, Southern Methodist University, 3215 Daniel Avenue, Dallas, TX 75275, USA}
\affiliation[42]{Sorbonne Universit\'{e}, CNRS/IN2P3, Laboratoire de Physique Nucl\'{e}aire et de Hautes Energies (LPNHE), FR-75005 Paris, France}
\affiliation[43]{Departament de F\'{i}sica, Serra H\'{u}nter, Universitat Aut\`{o}noma de Barcelona, 08193 Bellaterra (Barcelona), Spain}
\affiliation[44]{Department of Astronomy, The Ohio State University, 4055 McPherson Laboratory, 140 W 18th Avenue, Columbus, OH 43210, USA}
\affiliation[45]{Instituci\'{o} Catalana de Recerca i Estudis Avan\c{c}ats, Passeig de Llu\'{\i}s Companys, 23, 08010 Barcelona, Spain}
\affiliation[46]{Max Planck Institute for Extraterrestrial Physics, Gie\ss enbachstra\ss e 1, 85748 Garching, Germany}
\affiliation[47]{Department of Physics and Astronomy, Siena College, 515 Loudon Road, Loudonville, NY 12211, USA}
\affiliation[48]{Department of Physics \& Astronomy, University  of Wyoming, 1000 E. University, Dept.~3905, Laramie, WY 82071, USA}
\affiliation[49]{National Astronomical Observatories, Chinese Academy of Sciences, A20 Datun Rd., Chaoyang District, Beijing, 100012, P.R. China}
\affiliation[50]{Instituto Avanzado de Cosmolog\'{\i}a A.~C., San Marcos 11 - Atenas 202. Magdalena Contreras, 10720. Ciudad de M\'{e}xico, M\'{e}xico}
\affiliation[51]{Space Sciences Laboratory, University of California, Berkeley, 7 Gauss Way, Berkeley, CA  94720, USA}
\affiliation[52]{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}
\affiliation[53]{Universit\'{e} Clermont-Auvergne, CNRS, LPCA, 63000 Clermont-Ferrand, France}
\affiliation[54]{Department of Physics, Kansas State University, 116 Cardwell Hall, Manhattan, KS 66506, USA}
\affiliation[55]{Department of Physics \& Astronomy, Ohio University, Athens, OH 45701, USA}
\affiliation[56]{Department of Physics and Astronomy, Sejong University, Seoul, 143-747, Korea}
\affiliation[57]{Abastumani Astrophysical Observatory, Tbilisi, GE-0179, Georgia}
\affiliation[58]{Faculty of Natural Sciences and Medicine, Ilia State University, 0194 Tbilisi, Georgia}
\affiliation[59]{CIEMAT, Avenida Complutense 40, E-28040 Madrid, Spain}
\affiliation[60]{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}
\affiliation[61]{University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation[62]{Ecole Polytechnique F\'{e}d\'{e}rale de Lausanne, CH-1015 Lausanne, Switzerland}
\affiliation[63]{Department of Astronomy, Tsinghua University, 30 Shuangqing Road, Haidian District, Beijing, China, 100190}

